Generalized Hybrid Search and Applications to Blockchain and Hash Function Security

In this work we first examine the hardness of solving various search problems by hybrid quantum-classical strategies, namely, by algorithms that have both quantum and classical capabilities. We then construct a hybrid quantum-classical search algorithm and analyze its success probability. Regarding the former, for search problems that are allowed to have multiple solutions and in which the input is sampled according to arbitrary distributions we establish their hybrid quantum-classical query complexities -- i.e., given a fixed number of classical and quantum queries, determine what is the probability of solving the search task. At a technical level, our results generalize the framework for hybrid quantum-classical search algorithms proposed by Rosmanis. Namely, for an arbitrary distribution $D$ on Boolean functions, the probability an algorithm equipped with $\tau_c$ classical and $\tau_q$ quantum queries succeeds in finding a preimage of $1$ for a function sampled from $D$ is at most $\nu_D \cdot(2\sqrt{\tau_c} + 2\tau_q + 1)^2$, where $\nu_D$ captures the average (over $D$) fraction of preimages of $1$. As applications of our hardness results, we first revisit and generalize the security of the Bitcoin protocol called the Bitcoin backbone, to a setting where the adversary has both quantum and classical capabilities, presenting a new hybrid honest majority condition necessary for the protocol to properly operate. Secondly, we examine the generic security of hash functions against hybrid adversaries. Regarding our second contribution, we design a hybrid algorithm which first spends all of its classical queries and in the second stage runs a ``modified Grover'' where the initial state depends on the distribution $D$. We show how to analyze its success probability for arbitrary target distributions and, importantly, its optimality for the uniform and the Bernoulli distribution cases.

==> 6_Classical_Fourier_Analysis.tex <==
We will first introduce some notations and some useful results from Fourier boolean analysis.

\subsection{Background}

Let $f, g : \{-1, 1\}^n \rightarrow \mathbb{R}$.

Then, we define the inner product between the two functions as:
\begin{equation}
    \langle f, g \rangle := \frac{1}{2^n} \sum_{x \in \{-1, 1\}^n} f(x) \cdot g(x)
\end{equation}


We define the monomial corresponding to a subset $S \subseteq [n]$ as:
\begin{equation}
    x^S := \prod_{i \in S} x_i \ \ \ ; \ \ \ x^{\emptyset} = 1
\end{equation}

\begin{theorem}[Fourier Expansion]
    Every function $f : \{-1, 1\}^n \rightarrow \mathbb{R}$ can be uniquely expressed as a multilinear polynomial:
    \begin{equation}
        f(x) = \sum_{S \subseteq [n]} \hat{f}(S) \cdot x^S
    \end{equation}
    where the real number $\hat{f}(S)$ is called the Fourier coefficient of $f$ on $S$.
\end{theorem}

\begin{theorem} [Fourier Coefficient] \label{thm:fourier_coeff}
For any $f : \{-1, 1\}^n \rightarrow \mathbb{R}$ and for any subset $S \subseteq [n]$, the Fourier coefficient of $f$ on $S$ can be computed as:
\begin{equation}
    \hat{f}(S) = \langle f, x^S \rangle 
\end{equation}
    
\end{theorem}

\begin{theorem}[Inner Product] \label{thm:fourier_prod}
For any 2 functions $f, g: \{-1, 1\}^n \rightarrow \mathbb{R}$, the inner product of the Fourier coefficients is equal to the inner product of the two functions:
\begin{equation}
    \langle f, g \rangle = \sum_{S \subseteq [n]} \hat{f}(S) \cdot \hat{g}(S) 
\end{equation}
Hence, we have:
\begin{equation}
    \sum_{x \in \{-1, 1\}^n} f(x) \cdot g(x) = 2^n \sum_{S \subseteq [n]} \hat{f}(S) \cdot \hat{g}(S)
\end{equation}
\end{theorem}


\subsection{Analysis of General Classical Success}


In this section we will analyze and determine a general expression for the success probability of an arbitrary classical strategy for solving an arbitrary search problem - where the target boolean function is sampled according to an arbitrary distribution $\distr$.


We will denote the arbitrary classical strategy by a subset $S \subseteq [m]$ of size $\cquery$, $S := \{i_1, i_2, ..., i_{\cquery}\}$, denoting the indices of the classical queries performed during the search algorithm. In other words, the classical algorithm after the queries has the information: $(i_1, x_{i_1}), (i_2, x_{i_2}), \cdots, (i_{\cquery}, x_{i_{\cquery}})$.

As a result, it is clear that the algorithm failing to solve the search problem corresponds to the event where $x_{i_1} = x_{i_2} = \cdots = x_{i_{\cquery}} = 0$. \\
In other words if we define the function $g^S : \{0, 1\}^n \rightarrow \bool$, parameterized by the classical strategy $S$:
\begin{equation}
    g^S(x) := \prod_{j \in S} (1 - x_j)
\end{equation}
Then, we have that the probability of the failure of the classical algorithm $S$ corresponds to the probability that $g^S(x) = 1$.

We would like to analyze this probability using the boolean Fourier analysis framework, however first notice that for this we need to work with functions defined on $\{-1, 1\}$, instead of $\{0, 1\}$. This can be easily fixed by defining the function:
\begin{equation}
    \begin{split}
        \tilde{g}^S &: \{-1, 1\}^n \rightarrow \{0, 1\} \\
        \tilde{g}^S(z) &:= g^S \left(\frac{1 + z_1}{2}, \frac{1 + z_2}{2}, \cdots, \frac{1 + z_n}{2} \right) \\
        &= \frac{1}{2^\cquery} \prod_{j \in S} (1 - z_j)
    \end{split}
\end{equation}

Now, let us consider the function describing the target distribution $\distr$:
\begin{equation}
    \begin{split}
       & d : \bool^m \rightarrow [0, 1] \\
       & d(x) := \Pr_{x \leftarrow \distr}[x]
    \end{split}
\end{equation}
Similarly, we will define a function that acts exactly as $d$, but on the domain $\{-1, 1\}$:
\begin{equation}
    \begin{split}
        & \tilde{d} : \{-1, 1\}^m \rightarrow [0, 1] \\
        & \tilde{d}(z) := d \left(\frac{1 + z_1}{2}, \frac{1 + z_2}{2}, \cdots, \frac{1 + z_n}{2} \right)
    \end{split}
\end{equation}
Then, we can express the probability that the strategy $S$ fails as:
\begin{equation}
    \begin{split}
        \Pr^S[\mathsf{Classical \ Fail}] &= \Pr_{x \leftarrow D}[g^S(x) = 1] \\
                           &= \sum_{x \in \bool^m} d(x) \cdot g^S(x) \\
                           &= \sum_{x \in \bool^m} \tilde{d}(2x_1 - 1,\cdots, 2x_m - 1) \cdot \tilde{g}^S(2x_1 - 1,\cdots, 2x_m - 1) \\
                           &= \sum_{x \in \{-1, 1\}^m} \tilde{d}(x) \tilde{g}^S(x) 
    \end{split}
\end{equation}

And the \textbf{optimal} classical strategy is given by the strategy $S$ that minimizes $\Pr^S[\text{Fail}]$:
\begin{equation}
    \Pr[\mathsf{Classical \ Fail}] = \min_{S \subseteq [m]: |S| = \cquery}  \Pr^S[\mathsf{Classical \ Fail}]
\end{equation}

Now, using Theorem~\ref{thm:fourier_prod}, we can rewrite the failure probability as:
\begin{equation}
    \Pr^S[\text{Fail}] = 2^m \cdot \sum_{T \subseteq [m]} \widehat{\tilde{d}}(T) \cdot \widehat{{\tilde{g}^S}}(T)
\end{equation}
Using Theorem~\ref{thm:fourier_coeff}, we can further rewrite as:
\begin{equation}
    \Pr^S[\mathsf{Classical \ Fail}] = \frac{1}{2^m} \cdot \sum_{T \subseteq [m]} \left(\sum_{x \in \{-1, 1\}^m} \tilde{d}(x) \cdot \prod_{i \in T} x_i  \right) \left( \sum_{x \in \{-1, 1\}^m} \tilde{g}^S(x) \cdot \prod_{i \in T} x_i  \right)
\end{equation}


We notice that for the failure probability we have two functions: $\tilde{g}^S$ which only depends on the classical strategy and is independent of $\distr$ and $\tilde{d}$ which only depends on the target distribution $\distr$.

We can rewrite the failure probability as an expression only parameterized by the distribution function $\tilde{d}$ and in the following section, we will instantiate $d$ corresponding to specific target distributions.


\begin{equation} \label{eq:general_fail}
    \begin{split}
    \Pr^S[\mathsf{Classical \ Fail}] &= 
    \frac{1}{2^m} \cdot \sum_{T \subseteq [m]} \left(\sum_{x \in \{-1, 1\}^m} \tilde{d}(x) \cdot \prod_{i \in T} x_i  \right) \cdot \\
    & \ \ \ \ \ \ \ \ \ \cdot \left( \sum_{x \in \{-1, 1\}^m} \frac{1}{2^c} \cdot \prod_{j \in S} (1 - x_j) \cdot \prod_{i \in T} x_i \right) \\
    &= \frac{1}{2^m} \cdot \sum_{T \subseteq [m]} \left(\sum_{x \in \{-1, 1\}^m} \tilde{d}(x) \cdot \prod_{i \in T} x_i  \right) \cdot \left(  \sum_{x: x_{i_1} = \cdots = x_{i_c} = -1}  \prod_{i \in T} x_i \right)
    \end{split}
\end{equation}



We can rewrite $\Pr^S[\text{Fail}]$ as:
\begin{equation}
    \begin{split}
    \Pr^S[\text{Fail}]  &= \frac{1}{2^m} \sum_{T \subseteq S} \left[ \sum_{x \in \{-1, 1\}^m} \tilde{d}(x) \cdot \left(\prod_{i \in T} x_i\right) \right] \cdot \left[\sum_{x_{i_1} = x_{i_2} = ... = x_{i_c} = -1} \left( \prod_{i \in T} x_i \right) \right] \\
                        &= \frac{2^c}{2^m} \sum_{T \subseteq S} \frac{(-1)^{|T|}}{2^{|T|}} \cdot \sum_{x \in \{-1, 1\}^m} \tilde{d}(x) \cdot \left( \prod_{i \in T} x_i \right) \\
                        &= \frac{2^c}{2^m} \left( \sum_{x \in \{-1, 1\}^m} \tilde{d}(x) - \sum_{i_j \in S} \frac{1}{2} \sum_{x \in \{-1, 1\}^m} \tilde{d}(x) \cdot x_{i_j} \right) \\
                        & \ \ \ \ \ +  \frac{2^c}{2^m} \left(  \sum_{T \subseteq S: |T| \geq 2} \frac{(-1)^{|T|}}{2^{|T|}} \cdot \sum_{x \in \{-1, 1\}^m} \tilde{d}(x) \cdot \left( \prod_{i \in T} x_i \right) \right)  \\
                        &= \frac{2^c}{2^m} \left( 1 + \frac{c}{2} -  \sum_{i \in S} w(i) \right) \\
                        & \ \ \ \ \ +  \frac{2^c}{2^m} \left(  \sum_{T \subseteq S: |T| \geq 2} \frac{(-1)^{|T|}}{2^{|T|}} \cdot \sum_{x \in \{-1, 1\}^m} \tilde{d}(x) \cdot \left( \prod_{i \in T} x_i \right) \right)
    \end{split}
\end{equation}

\subsection{Classical Success for Particular Distributions}

In previous section, we have established the failure probability as a function of the target distribution $\distr$. In this part, we will instantiate the function $d$ according to specific choices of distributions.


\subsubsection{Uniform Distribution}

Let $\distr$ be the distribution which samples uniformly at random from all the functions $f : \bool^m \rightarrow \bool$ which has a unique preimage of $1$.

\begin{lemma}[Uniform Classical Success] \label{lemma:uniform_classical_sucess}
      For $\distr$ the uniform distribution, the probability of success of any classical algorithm equipped with $\cquery$ classical queries is equal to:
      \begin{equation}
    \Pr[\mathsf{Classical \ Succcess}] = \frac{\cquery}{m}
    \end{equation}
\end{lemma}

\begin{proof}
This corresponds to the distribution function $\tilde{d} : \{-1, 1\}^m \rightarrow [0, 1]$:
\begin{equation}
    \tilde{d}(x) = 
    \begin{cases}
        & \frac{1}{m} \ , \ \text{if } \mathsf{hw}(x) = 1 \\
        & 0 \ , \ \text{otherwise}
    \end{cases}
\end{equation}
where $\mathsf{hw} : \{-1, 1\}^m \rightarrow \mathbb{Z}$, $\mathsf{hw}(x)$ outputs the number of indices $i$ for which $x_i = 1$. 

Using the definition of $d$ and Equation~(\ref{eq:general_fail}) we have:
\begin{equation}
    \begin{split}
    \Pr^S[\mathsf{Classical \ Fail}] &= \frac{1}{2^m} \cdot \frac{1}{m} \cdot \sum_{T \subseteq [m]} \left[ \sum_{x :  \mathsf{hw}(x) = 1} \left( \prod_{i \in T} x_i \right) \right] \cdot \\
    & \ \ \ \ \ \ \cdot \left[ \sum_{x : x_{i_1} = \cdots = x_{i_{\cquery}} = -1} \left( \prod_{i \in T} x_i \right) \right] \\
    &= \frac{1}{2^m \cdot m} \sum_{T \subseteq [m]} A_T \cdot B_T
    \end{split}
\end{equation}
Let us analyze this expression by computing the sum for each possible size of $T$:
\begin{itemize}
    \item $T = \emptyset$: $A_T \cdot B_T = m \cdot 2^{m - \cquery}$;
    
    \item $|T| = 1$. Let $T = \{j\}$. 
    \begin{enumerate}
        \item  If $j \in S$, then $x_j = -1$;
        \item  Else if $j \not\in S$, we have that $B_T = \sum_{x : x_{i_1} = \cdots = x_{i_{\cquery}} = -1} x_j = 0$;
    \end{enumerate}
    Hence we have: $A_T \cdot B_T = (1 - (m - 1)) \cdot (-1) 2^{m - \cquery}$
    
    \item $|T| = 2$. Let $T = \{j_1, j_2\}$. Then:
    \begin{enumerate}
        \item If $j_1, j_2 \in S$ we have $B_T = (-1) \cdot (-1) \cdot 2^{m - \cquery}$;
        \item If $j_1 \not\in S$ or $j_2 \not\in S$, we have: $B_t = 0$;
    \end{enumerate}
    Therefore $A_T \cdot B_T = (2 \cdot (-1) + m - 2)(-1) \cdot (-1) \cdot 2^{m - \cquery} = (m - 4) 2^{m - \cquery}$
    \item For $|T| = k$, where $k \leq \cquery$, it can be shown similarly that:
    \begin{equation}
        A_T \cdot B_T = 2^{m - \cquery} \cdot (m - 2k)
    \end{equation}
\end{itemize}
Now, to derive the failure probability we need to combine these expressions. One important observation is that for each possible size $k$ of $T$, the number of such sets that would contribute to the sum ($\Pr^S[\text{Fail}]$) are those sets $T$ that are subsets of $S$, as otherwise if $S \not\subseteq S$, we have: $B_T = 0$. Hence the number of such subsets $T$ is equal to: 
%$|\{ T \subseteq [m]: |T| = k \text{ and } T \subseteq S \}| = {\cquery \choose k}$.
$|\{ T \subseteq [m]: |T| = k \text{ and } T \subseteq S \}| = \binom{\cquery}{k}$.
Therefore, we get:
\begin{equation}
    \begin{split}
     \Pr^S[\mathsf{Classical \ Fail}] &=  \frac{1}{2^m} \cdot \frac{1}{m} \sum_{T \subseteq [m]} A_T \cdot B_T \\
        &= \frac{1}{2^m} \cdot \frac{1}{m} \left[2^{m - \cquery} \cdot m \cdot {m \choose 0} + 2^{m - \cquery} \cdot (m - 2) \cdot {m \choose 1} + \cdots + \right. \\
        & \left. \ \ \ \ \ \ \ + 2^{m - \cquery} (m - 2\cquery) \cdot {m \choose \cquery} \right] \\
        &= \frac{1}{m} \cdot \frac{1}{2^{\cquery}} \sum_{k = 0}^{\cquery} (m - 2 \cdot k) \cdot {\cquery \choose k} \\
        &= \frac{1}{m} \cdot \frac{1}{2^{\cquery}} \left[m \cdot \left( \sum_{k = 0}^{\cquery} {\cquery \choose k} \right) - 2 \cdot \left(\sum_{k = 0}^{\cquery} k \cdot {\cquery \choose k} \right) \right] \\
        &= \frac{1}{m} \cdot \frac{1}{2^{\cquery}} \left(m \cdot 2^{\cquery} - 2 \cdot 2^{\cquery - 1} \cdot \cquery \right) \\
        &= 1 - \frac{2^{\cquery} \cdot \cquery}{m \cdot 2^{\cquery}} = 1 - \frac{\cquery}{m}
    \end{split} 
\end{equation}
This shows that for any strategy $S$ we have exactly the same probability of failure and hence the probability of success for any classical strategy using $\cquery$ classical queries is exactly:
\begin{equation}
    \Pr[\mathsf{Classical \ Success}] = 1 - \Pr^S[\mathsf{Classical \ Fail}] = \frac{\cquery}{m}
\end{equation}
\end{proof}


\subsubsection{Bernoulli Distribution}

\begin{lemma}[Bernoulli Classical Success] \label{lemma:bernoulli_classical_sucess}
      For $\distr$ the Bernoulli distribution parameterized by $\eta$, the probability of success of any classical algorithm equipped with $\cquery$ classical queries is equal to:
      \begin{equation}
    \Pr[\mathsf{Classical \ Success}] =  1 - (1 - \eta)^{\cquery}
    \end{equation}
\end{lemma}

\begin{proof}

In this part we are dealing with search problems for which we have:
$$ \Pr[x_i = 1] = \eta \ \ \ \text{for all } i \in [m] $$

As a result, we have the distribution function:
\begin{equation}
    \tilde{d}(x) = \eta^{\mathsf{hw}(x)} \cdot (1 - \eta)^{m - \mathsf{hw}(x)}
\end{equation}

Using this definition and Equation~(\ref{eq:general_fail}) we have:
\begin{equation}
    \begin{split}
    \Pr^S[\mathsf{Classical \ Fail}] &= \frac{1}{2^m} \sum_{T \subseteq [m]} \left[ \sum_{x \in \{-1, 1\}^m} \tilde{d}(x) \left(\prod_{i \in T} x_i\right) \right] \cdot \\
    & \ \ \ \ \ \ \ \cdot \left[ \sum_{x : x_{i_1} = \cdots = x_{i_{\cquery}} = -1} \left( \prod_{i \in T} x_i \right) \right] \\
    &=  \frac{1}{2^m} \cdot \sum_{T \subseteq [m]} A_T \cdot B_T
    \end{split}
\end{equation}

Let us analyze this expression by computing the sum for each possible size of $T$:
\begin{itemize}
    \item $T = \emptyset$: 
    \begin{equation}
        \begin{split}
        A_T \cdot B_T &= \left[ \sum_{x : \mathsf{hw}(x) = 0} (1 - \eta)^m + \sum_{x : \mathsf{hw}(x) = 1} \eta \cdot (1 - \eta)^{m - 1} + \cdots + \sum_{x : \mathsf{hw}(x) = m} \eta^m \right] \cdot \\  
        & \ \ \ \ \ \ \ \cdot \sum_{x : x_{i_1} = \cdots = x_{i_{\cquery}} = -1} 1  \\
        &= \left[{m \choose 0} (1 - \eta)^m + {m \choose 1}\eta \cdot (1 - \eta)^{m - 1} + \cdots {m \choose m}  \eta^m  \right] \cdot 2^{m - \cquery} \\
        &= (1 - \eta + \eta)^m \cdot 2^{m - \cquery} = 2^{m - \cquery}
        \end{split}
    \end{equation}
    
    \item $|T| = 1$. Let $T = \{j\}$. 
    \begin{enumerate}
        \item  If $j \in S$, then $x_j = -1$;
        \item  Else if $j \not\in S$, we have that $B_T = \sum_{x : x_{i_1} = \cdots = x_{i_{\cquery}} = -1} x_j = 0$;
    \end{enumerate}
    Hence we have: 
    \begin{equation}
        A_T \cdot B_T = \left( \sum_{z \in \{-1, 1\}^m} \tilde{d}(z) \cdot z_j \right) \cdot \left(-2^{m - \cquery} \right)  
    \end{equation}
We will split $A_T$ into $m$ terms corresponding to all possible Hamming weights: $A_T = A_0 + \cdots A_m$, where $A_i := \sum_{z \in \{-1, 1\}^m: \mathsf{hw}(z) = i} \tilde{d}(z) \cdot z_j$. Then, we have:
\begin{equation}
    A_0 = (1 - \eta)^m (-1) \cdot 1
\end{equation}
\begin{equation}
    \begin{split}
    A_1 &= \eta (1 - \eta)^{m - 1} \sum_{z: \mathsf{hw}(z) = 1} z_j \\
    &= \eta \cdot (1 - \eta)^{m - 1} \left( \sum_{z: \mathsf{hw}(z) = 1 , z_j = 1 } z_j  + \sum_{z: \mathsf{hw}(z) = 1 , z_j = -1 } z_j  \right) \\
    &= \eta \cdot (1 - \eta)^{m - 1} \left(1 \cdot {m - 1 \choose 0} + (-1) \cdot {m - 1 \choose 1}\right)
    \end{split}
\end{equation}
\begin{equation}
    \begin{split}
    A_2 &= \eta^2 (1 - \eta)^{m - 2} \sum_{z: \mathsf{hw}(z) = 2} z_j \\
     &= \eta^2 \cdot (1 - \eta)^{m - 2} \left( \sum_{z: \mathsf{hw}(z) = 2 , z_j = 1 } z_j  + \sum_{z: \mathsf{hw}(z) = 2 , z_j = -1 } z_j  \right) \\
     &= \eta^2 \cdot (1 - \eta)^{m - 2} \left(1 \cdot {m - 1 \choose 1} + (-1) \cdot {m - 1 \choose 2}\right)
    \end{split}
\end{equation}
For any $i \in [m - 1]$:
\begin{equation}
    A_i = \eta^i \cdot (1 - \eta)^{m - i} \cdot \left[ {m - 1 \choose i - 1} - {m - 1 \choose i} \right]
\end{equation}
\begin{equation}
    A_m = \eta^m \sum_{z \in \{-1, 1\}^m: \mathsf{hw}(z) = m} z_j = \eta^m 
\end{equation}

As a result, by combining the above, we get:
\begin{equation}
    \begin{split}
        A_T &= A_0 + A_1 + \cdots + A_m \\
        &= - (1 - \eta)^m \cdot {m - 1 \choose 0} +  \eta^m \cdot {m - 1 \choose m - 1} \\
        & \ \ \ \ \ \ + \left[ \sum_{i = 1}^{m - 1} \eta^i \cdot (1 - \eta)^{m - i} \cdot \left( {m - 1 \choose i - 1} - {m - 1 \choose i} \right) \right] \\
        &= {m - 1 \choose 0} \left[\eta \cdot (1 - \eta)^{m - 1} - (1 - \eta)^m  \right] + \\
        & \ \ \ \ + {m - 1 \choose 1} \left[\eta^2 (1 - \eta)^{m - 2} - \eta (1 - \eta)^{m - 1}  \right] + \cdots + \\
        %&+ {m - 1 \choose m - 2} \left[\eta^{m - 1} \cdot (1 - \eta) - \eta^{m - 2} \cdot (1 - \eta)^2  \right] +
        & \ \ \ \  + {m - 1 \choose m - 1} \left[\eta^m - \eta^{m - 1} \cdot (1 - \eta)  \right] \\
        &= \sum_{i = 0}^{m - 1} {m - 1 \choose i} \left[ \eta^{i + 1} (1 - \eta)^{m - i - 1} - \eta^i (1 - \eta)^{m - i} \right] \\
        &= \sum_{i = 0}^{m - 1} {m - 1 \choose i} \eta^i (1 - \eta)^{m - i - 1} (2 \eta - 1) \\
        &= (2 \eta - 1) \cdot (\eta + 1 - \eta)^{m - 1} = 2 \eta - 1
    \end{split}
\end{equation}

\begin{equation}
    A_T \cdot B_T = 2^{m - \cquery} (1 - 2\eta)
\end{equation}



    \item $|T| = 2$. Let $T = \{j_1, j_2\}$. \\
    \begin{enumerate}
        \item If $j_1, j_2 \in S$ we have $B_T = (-1) \cdot (-1) \cdot 2^{m - \cquery}$;
        \item If $j_1 \not\in S$ or $j_2 \not\in S$, we have: $B_t = 0$;
    \end{enumerate}

\begin{equation}
    \begin{split}
        A_T \cdot B_T &= \left( \sum_{z \in \{-1, 1\}^m} \tilde{d}(z) \cdot z_j \right) \cdot \left( \sum_{x_{i_1} = ... = x_{i_{\cquery}} = -1} x_{j_1} x_{j_2}\right) \\
        &= 2^{m - \cquery} \cdot \left[ \sum_{i = 0}^m \sum_{z \in \{-1, 1\}^m: \mathsf{hw}(z) = i} (1 - \eta)^{m - i} \eta^i \cdot z_{j_1} \cdot z_{j_2} \right]
    \end{split}
\end{equation}
    As before we analyze separately for each possible value of the hamming weight. Namely, we define:
    \begin{equation}
        A_i = \sum_{z \in \{-1, 1\}^m: \mathsf{hw}(z) = i} (1 - \eta)^{m - i} \eta^i \cdot z_{j_1} \cdot z_{j_2}
    \end{equation}

\begin{equation}
    A_0 = \sum_{z : \mathsf{hw}(z) = 0} (1 - \eta)^{m} \cdot z_{j_1} \cdot z_{j_2} = (1 - \eta)^{m}
\end{equation}
\begin{equation}
    A_m = \sum_{z : \mathsf{hw}(z) = m} \eta^{m} \cdot z_{j_1} \cdot z_{j_2} = \eta^{m}
\end{equation}

\begin{equation}
    \begin{split}
     A_1 &= \sum_{z : \mathsf{hw}(z) = 1} (1 - \eta)^{m - 1} \cdot \eta \cdot z_{j_1} \cdot z_{j_2} \\
     &= (1 - \eta)^{m - 1} \cdot \eta \cdot \left[ 
        \sum_{\substack{z : \mathsf{hw}(z) = 1 \\ z_{j_1} = 1, z_{j_2} = -1}} z_{j_1} \cdot z_{j_2} + 
        \sum_{\substack{z : \mathsf{hw}(z) = 1 \\ z_{j_1} = -1, z_{j_2} = 1}} z_{j_1} \cdot z_{j_2} + \right. \\
       & \left. \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  + \sum_{\substack{z : \mathsf{hw}(z) = 1 \\ z_{j_1} = -1, z_{j_2} = -1}} z_{j_1} \cdot z_{j_2}
     \right] \\
     &= (1 - \eta)^{m - 1} \cdot \eta \cdot \left[ 2 \cdot (-1) \cdot 1 + (-1) \cdot (-1) \cdot {m - 2 \choose 1} \right]
    \end{split}
\end{equation}
\begin{equation}
    \begin{split}
         A_2 &= \sum_{z : \mathsf{hw}(z) = 2} (1 - \eta)^{m - 2} \cdot \eta^2 \cdot z_{j_1} \cdot z_{j_2} \\
         &=  (1 - \eta)^{m - 2} \eta^2 \left[
            \sum_{\substack{z : \mathsf{hw}(z) = 2 \\ z_{j_1} = 1, z_{j_2} = 1}} z_{j_1} \cdot z_{j_2} +
            \sum_{\substack{z : \mathsf{hw}(z) = 2 \\ z_{j_1} = 1, z_{j_2} = -1}} z_{j_1} \cdot z_{j_2} + \right. \\
           & \left. \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  + \sum_{\substack{z : \mathsf{hw}(z) = 2 \\ z_{j_1} = -1, z_{j_2} = 1}} z_{j_1} \cdot z_{j_2} + 
            \sum_{\substack{z : \mathsf{hw}(z) = 2 \\ z_{j_1} = -1, z_{j_2} = -1}} z_{j_1} \cdot z_{j_2}
         \right] \\
         &= (1 - \eta)^{m - 2} \eta^2 \left[ 1 \cdot 1 \cdot 1 \cdot 1 + 2 \cdot 1 \cdot (-1) \cdot {m - 2 \choose 1} + \right. \\
          & \left. \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  + (-1) \cdot (-1) \cdot {m - 2 \choose 2} \right]
    \end{split} 
\end{equation}
\begin{equation}
    A_{m - 2} = (1 - \eta)^2 \eta^{m - 2} \left[ {m - 2 \choose m - 4} - 2 \cdot {m - 2 \choose m - 3} + {m - 2 \choose m - 2} \right]
\end{equation}

\begin{equation}
    A_{m - 1} = (1 - \eta) \eta^{m - 1} \left[ {m - 2 \choose m - 3} - 2 \cdot {m - 2 \choose m - 2} \right]
\end{equation}
Then by combining these results we obtain:
\begin{equation}
    \begin{split}
    A_T &= \sum_{i = 0}^m A_i \\
        &= {m - 2 \choose 0}  \left[ (1 - \eta)^m - 2 (1 - \eta)^{m - 1} \eta + (1 - \eta)^{m - 2} \eta^2 \right] + \\
        & \ \ \ \ \ \ + {m - 2 \choose 1} [ (1 - \eta)^{m-1} \eta - 2 (1 - \eta)^{m - 2} \eta^2 + (1 - \eta)^{m - 3} \eta^3 ] + \cdots + \\ 
        %&+ {m - 2 \choose m - 3} \left[ (1 - \eta)^3 \eta^{m - 3} - 2 (1 - \eta)^{2} \eta^{m - 2} + (1 - \eta) \eta^{m - 1} \right] +
        & \ \ \ \ \ \ + {m - 2 \choose m - 2} \left[ (1 - \eta)^2 \eta^{m - 2} - 2 (1 - \eta) \eta^{m - 1} + \eta^m \right] \\
        &= (1 - 2 \eta)^2 \left[{m - 2 \choose 0} \cdot (1 - \eta)^{m - 2} + {m - 2 \choose 1} \cdot (1 - \eta)^{m - 3} \eta + \cdots + \right. \\
        &\left. \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  + {m - 2 \choose m - 2} \eta^{m - 2} \right] \\
        &= (1 - 2 \eta)^2 \left[(1 - \eta + \eta)^{m - 2} \right] = (1 - 2\eta)^2
        \end{split}
\end{equation}

% {\substack{1\le i\le n\\ i\ne j}}    
    Therefore $A_T \cdot B_T =  2^{m - \cquery} (1 - 2\eta)^2$.


    \item For $|T| = k$, where $k \leq \cquery$, it can be shown similarly that:
    \begin{equation}
        A_T \cdot B_T = 2^{m - \cquery} (1 - 2\eta)^k
    \end{equation}
\end{itemize}

The final probability of failure can be expressed as:
\begin{equation}
    \Pr[\mathsf{Classical \ Fail}] = \frac{1}{2^m} \left[P_{T = \emptyset} + P_{|T| = 1} + \cdots + P_{|T| = \cquery}  \right]
\end{equation}
where $P_{|T| = k} = A_T \cdot B_T \cdot |\{ T \subseteq [m]: |T| = k \text{ and } T \subseteq S \}|$.

As a result, we conclude that:
\begin{equation}
    \begin{split}
     \Pr[\mathsf{Classical \ Fail}] &= \frac{1}{2^m} \left[ \sum_{k = 0}^{\cquery} 2^{m - \cquery}  (1 - 2\eta)^k {\cquery \choose k} \right] \\
     &= \frac{1}{2^{\cquery}} \left[\sum_{k = 0}^{\cquery} (1 - 2\eta)^k 1^{\cquery - k} \right] \\
     &= \frac{1}{2^{\cquery}} (1 - 2\eta + 1)^{\cquery} = (1 - \eta)^{\cquery}
    \end{split}
\end{equation}
And therefore, this also implies that for any strategy $S$ performing $\cquery$ classical queries the success probability is always equal to:
\begin{equation}
     \Pr[\mathsf{Classical \ Success}] = 1 - (1 - \eta)^{\cquery}
\end{equation}

    
\end{proof}


==> macros.tex <==
%!TEX root = rational.tex

\RequirePackage{amsopn}
\RequirePackage{ifthen}
\RequirePackage{xcolor}




%----------note----------%
\def\showauthnotes{1}
\ifthenelse{\showauthnotes=1}
{
\newcommand{\authnote}[2]{[{\color{blue}\textbf{#1:}}~{\color{blue} #2}]}
}
{ \newcommand{\authnote}[2]{} 
}

\newcommand{\fsnote}[1]{\authnote{FS}{#1}}
\newcommand{\jnote}[1]{\authnote{JG}{#1}}
\newcommand{\Cojo}[1]{\authnote{AC}{#1}}


\newcommand{\new}[1]{\textcolor{red}{#1}}



\renewcommand{\paragraph}[1]{\medskip\noindent{\bf #1}}

\newenvironment{nffunc}[3][]{
\begin{center}
   \begin{tabular}{|ll|}\hline
     \hspace{.3ex}\begin{minipage}{.92\linewidth}\vspace{0.5ex}
       {\begin{center}{\bf Functionality} #2 \end{center}}\vspace{-2ex}#3 \begin{itemize}%\setlength{\itemsep}{0mm} \setlength{\parskip}{0pt}
% \setlength{\parsep}{0pt}
\vspace{-1ex}%\vspace{-3ex}
       }{%
       \end{itemize}
       \vspace{-1ex}
       \smallskip
     \end{minipage}& \\
     \hline
   \end{tabular}
   \end{center}
}


\newenvironment{vnffunc}[3][]{
\begin{center}
   \begin{tabular}{|ll|}\hline
     \hspace{.3ex}\begin{minipage}{.92\linewidth}\vspace{0.5ex}
       {\begin{center}{\bf Functionality} #2 \end{center}}\vspace{-2ex}#3 %\begin{itemize}%\setlength{\itemsep}{0mm} \setlength{\parskip}{0pt}
% \setlength{\parsep}{0pt}
%\vspace{1ex}%\vspace{-3ex}
       }{%
       %\end{itemize}
       %\vspace{-1ex}
       \smallskip
     \end{minipage}& \\
     \hline
   \end{tabular}
   \end{center}
}




\newenvironment{nff}[3][]{
\begin{center}
   \begin{tabular}{|ll|}\hline
     \hspace{.3ex}\begin{minipage}{.92\linewidth}\vspace{0.5ex}
       {\begin{center}{} #2 \end{center}}\vspace{-2ex}#3 \begin{itemize}%\setlength{\itemsep}{0mm} \setlength{\parskip}{0pt}
% \setlength{\parsep}{0pt}
\vspace{-1ex}%\vspace{-3ex}
       }{%
       \end{itemize}
       \vspace{-1ex}
       \smallskip
     \end{minipage}& \\
     \hline
   \end{tabular}
   \end{center}
}



\newenvironment{nfprot}[3][]{
\begin{center}\small
  \begin{tabular}{|ll|}\hline
        \hspace{.3ex}\begin{minipage}{.95\linewidth}\vspace{0.5ex}
          {\begin{center}{\bf Protocol} #2 \end{center}}\vspace{-2ex}#3 % \begin{enumerate}\setlength{\itemsep}{2mm} \setlength{\parskip}{0pt}
% \setlength{\parsep}{0pt}
%\vspace{-1ex}%\vspace{-3ex}
          }{%
%          \end{enumerate}
          \vspace{-1ex}
          \smallskip
        \end{minipage}& \\
        \hline
  \end{tabular}
  \end{center}    \vspace{-1ex}
}

\newenvironment{inbox}%
{
    \begin{tabular}{|ll|}\hline\hspace{.3ex}
    \begin{minipage}{.85\linewidth}\vspace{0.5ex}
}%
{
    \vspace{0.5ex}
    \end{minipage}& \\
    \hline
    \end{tabular}
}


\newenvironment{protocol}[2][Protocol]{%
  % \setlength{\tabcolsep}{.7em}
  \begin{center}
    \begin{tabular}{|l|}\hline
      \begin{minipage}{.99\linewidth}\vspace{.1ex}
        \subsubsection*{#1 #2} \begin{enumerate}
        }{%
        \end{enumerate}\vspace{-.5ex}
        \vspace{-1.5ex} \smallskip
      \end{minipage}\\ %\ \vspace{-.5ex}
      \hline
    \end{tabular}
  \end{center}
}

\def\changemargin#1#2{\list{}{\rightmargin#2\leftmargin#1}\item[]}
\let\endchangemargin=\endlist 




% The set of all possible views does not depend on the environment and simulator, but it is easy to convert this back by just changing the command:
%\newcommand{\Fview}{\iview^{\frel}_{\frel,\Sim,\env}}
\newcommand{\Fview}{\iview_{\frel}}
\newcommand{\Zview}{\iview_{\env}}


\newcommand{\adv}{\ensuremath{\mathcal{A}}\xspace}
\newcommand{\dum}{\ensuremath{\mathcal{D}}\xspace}
\newcommand{\dist}{\ensuremath{\mathcal{D}}\xspace}
%\newcommand{\abortAdv}{\ensuremath{\adv_\dagger}\xspace}
\newcommand{\abortAdv}{\ensuremath{\adv_{\rm gen}}\xspace}
\newcommand{\algo}{\mathcal{B}}
\newcommand{\env}{\ensuremath{\mathcal{Z}}\xspace}
\newcommand{\func}[1][\relax]{\ensuremath{\mathcal{F}_{\textsc{#1}}}\xspace}
%\newcommand{\fsfe}{\func{SFE}}
\newcommand{\PH}{\mathcal{H}}
\newcommand{\D}{\ensuremath{D}\xspace}
\newcommand{\M}{\ensuremath{\mathcal{M}}\xspace}
\renewcommand{\sim}{\ensuremath{\mathcal{S}}\xspace}
\newcommand{\nt}[1]{\ensuremath{[#1]}\xspace}
%\newcommand{\exec}{\ensuremath{{\sf Exec}}\xspace}
\newcommand{\exec}{\ensuremath{\textsc{exec}}\xspace}
\newcommand{\indist}[1][\relax]{\ensuremath{\overset {#1}{\approx}}}
\newcommand{\negeq}{\ensuremath{\mathrel{\accentset{\ \mathsf{negl}}{\mathop\approx}}}}
\newcommand{\neglgeq}{\mathrel{\accentset{\ \mathsf{negl}}{\mathop\geq}}}
\newcommand{\neglleq}{\mathrel{\accentset{\ \mathsf{negl}}{\mathop\leq}}}
\newcommand{\neglle}{<}
\newcommand{\neglge}{>}

\newcommand{\tconst}{\ensuremath{\delta}}
\newcommand{\econst}[1][\relax]{\ensuremath{\epsilon_{#1}}\xspace}


%%%% Such that we can easily switch between greedy and rational
\newcommand{\rational}{rational\xspace}
\newcommand{\Rational}{Rational\xspace}
%%%% Such that we can easily switch between greedy and rational

%\newcommand{\RGS}{PG\xspace}
\newcommand{\RGS}{HG\xspace}
\newcommand{\com}[1][\relax]{\ensuremath{\mathsf{com}_{#1}}\xspace}
\newcommand{\dec}[1][\relax]{\ensuremath{\mathsf{dec}_{#1}}\xspace}
\newcommand{\skey}[1][\relax]{\ensuremath{\mathsf{sk}_{#1}}\xspace}
\newcommand{\pkey}[1][\relax]{\ensuremath{\mathsf{pk}_{#1}}\xspace}
\newcommand{\ok}{\ensuremath{\mathsf{ok}}\xspace}
\newcommand{\nok}{\ensuremath{\mathsf{nok}}\xspace}
\newcommand{\CA}{\ensuremath{\mathcal{L}_A}\xspace}

\newcommand{\cancel}[1]{}
\newcommand{\prp}{\ensuremath{{\tt ProbRelease}}\xspace}
\newcommand{\pitwo}{\ensuremath{{\tt \Pi}_2}\xspace}
%\newcommand{\pitwosfe}{\ensuremath{{\tt \pi}_{2SFE}}\xspace}
\newcommand{\pitwosfe}{\ensuremath{{\tt \Pi}_{\tt Op-SFE}}\xspace}
\newcommand{\prsfe}{\ensuremath{{\tt \Pi}_{\tt SFE}}\xspace}
%\newcommand{\prc}{\ensuremath{{\tt \pi}_{R\-2PC}}\xspace}
\newcommand{\prc}{\ensuremath{{\tt \Pi}_{\rm PFRC}}\xspace}
\newcommand{\pbot}{\ensuremath{{\tt \Pi}_\bot}\xspace}
\newcommand{\Sims}{\mathbb{S}}
\newcommand{\Sim}{\ensuremath{\mathcal{S}}\xspace}
\newcommand{\dummy}{\ensuremath{\mathcal{D}}\xspace}
\newcommand{\R}{\mathcal{R}}
\newcommand{\prd}{\ensuremath{\mathcal{D}}\xspace}
\newcommand{\prca}{\ensuremath{\mathcal{D_{\CA}}}\xspace}
\newcommand{\optp}{\ensuremath{\mathcal{P}}\xspace}
%\newcommand{\defeq}{\stackrel{\text{def}}{=}}
%\newcommand{\defeq}{\stackrel{\triangle}{=}}
%\newcommand{\ignore}[1]{}
\newcommand{\frelk}{\ensuremath{\mathcal{\frel[{\func[K07]}]}}\xspace}
%\newcommand{\pistate}{\ensuremath{\vec{\mathcal{S}}}\xspace}
\newcommand{\pistate}{\ensuremath{\vec{S}}\xspace}
\newcommand{\prel}{\bar\pi}
\newcommand{\prot}{\ensuremath{\Pi}\xspace}
\newcommand{\sh}[1]{\ensuremath{\langle #1\rangle}\xspace}
\newcommand{\funsh}[1][\relax]{\ensuremath{f_{{\rm sh},#1}}\xspace}
\newcommand{\fsh}{\func[sh]}
\newcommand{\fbc}{\func[bc]}
\newcommand{\fcf}[1][\relax]{\ensuremath{\func[CExch]^{#1}}\xspace}
%\newcommand{\ftf}{\ensuremath{{\func[2EX]}^\bot}\xspace}
\newcommand{\ftf}{\ensuremath{{{\mathcal F}_{\rm 2Ex}^\bot}}\xspace}
\newcommand{\fcom}{\func[com]}
\newcommand{\fauth}{\func[auth]}
\newcommand{\fabort}{\ensuremath{\func^\perp}\xspace}
\newcommand{\fclock}{\func[clock]}
\newcommand{\fcsfe}[1][\relax]{\ensuremath{\func[com-sfe]^{#1}}\xspace}
\newcommand{\fsfe}[1][\relax]{\ensuremath{\func[sfe]^{#1}}\xspace}
\newcommand{\frelsfe}[1][\relax]{\ensuremath{\frel[{\fsfe[#1]}]}\xspace}
\newcommand{\fmpc}[1][\relax]{\ensuremath{\func[rc]^{#1}}\xspace}
\newcommand{\fsfeNF}[1]{\fsfe[\bot,#1]}
\newcommand{\fsmt}{\func[smt]}
\newcommand{\frel}[1][\ensuremath{\mathcal{F}}]{\ensuremath{\langle #1 \rangle}\xspace}
\newcommand{\fdist}{\func[rr]^{\recon}}
\newcommand{\fid}{\ensuremath{f_{\sf swp}}\xspace}
\newcommand{\vsm}[1]{\ensuremath{\tilde{#1}}\xspace}
\newcommand{\vsmset}[1]{\ensuremath{\{\cup\vsm{#1}\}}\xspace}
\newcommand{\defeq}{\stackrel{\mathrm{def}}{=}}


\newcommand{\selParty}{\mathsf{sel}}
\newcommand{\rnd}{\mathsf{rnd}}
\newcommand{\aux}{\mathsf{aux}}
\newcommand{\poly}{\mathsf{poly}}
\newcommand{\sharegen}{\textnormal{\textsf{ShareGen}}}


\newcommand{\vparty}{\ensuremath{P}\xspace}

\newcommand{\rrProt}[1][\relax]{\Pi_\textsc{rr}^{#1}}

\newcommand{\set}[1]{\mathcal{#1}}
\newcommand{\HO}{\set{H}}
\newcommand{\PS}{\ensuremath{\set{P}}\xspace}
\newcommand{\F}{\ensuremath{\mathbb{F}}\xspace}

\newcommand{\ratio}{\varrho}
\newcommand{\round}{l}
\newcommand{\rdist}{\mathcal{D}}


\newcommand{\etwopc}[1]{\ensuremath{E_{#1}^{\rm R}}\xspace}
\newcommand{\empc}[1]{\ensuremath{E_{#1}^{\rm MPC}}\xspace}


\newcommand{\erel}[1]{\ensuremath{E_{#1}^{\tt Real}}\xspace}

\newcommand{\etwopcl}[1]{\ensuremath{E_{#1}^{\tt R,\lambda}}\xspace}

\newcommand{\etwopclr}[1]{\ensuremath{E_{#1}^{\tt R,\lambda,\rho}}\xspace}

\DeclareMathOperator{\argmin}{argmin}
\DeclareMathOperator{\diff}{d}
\newcommand{\reals}{\mathbb{R}}

\newcommand{\coloneqq}{\mathrel:\joinrel=}
\newcommand{\assign}{\coloneqq}
\newcommand{\dotcup}{\accentset{\cdot}{\cup}}
\newcommand{\natint}{\mathbf{N}}
\newcommand{\vcom}{\ensuremath{{\tt Com}}}
\newcommand{\vdec}{\ensuremath{{\tt Dec}}}


\newcommand{\corruptthreshold}{\alpha}
\newcommand{\cmd}[1]{\ensuremath{\textnormal{\texttt{#1}}}\xspace}
\newcommand{\vabort}{\cmd{abort}}
\newcommand{\vactivated}{\cmd{activated}}
\newcommand{\vcorrupt}{\cmd{corrupt}}
\newcommand{\vearly}{\cmd{early}}
\newcommand{\vinput}{\cmd{input}}
\newcommand{\voutput}{\cmd{output}}
\newcommand{\vpartial}{\cmd{partial}}
\newcommand{\vready}{\cmd{ready}}
\newcommand{\pgain}[1]{\ensuremath{\textsc{Prot-Gain}_{#1}}}
\newcommand{\degfair}[1]{\ensuremath{\textsc{Deg-Fair}_{#1}}}

\newcommand{\furnd}{\ensuremath{Rnd}\xspace}
%\newcommand{\again{\texttt{rscore}}\xspace}
%\newcommand{\realscoretxt}{\ensuremath{\textnormal{\textsf{rscore}}}}
\newcommand{\realscoretxt}[1][\relax]{\ensuremath{{U^{#1}}}}
%\newcommand{\realscoretxt}[1][\relax]{\ensuremath{{U_R^{#1}}}}
\newcommand{\idealscoretxt}[1][\relax]{\ensuremath{{U^{#1}_I}}}
\newcommand{\realscorefairtxt}{\ensuremath{\textnormal{\textsf{rscore}}_{\textnormal{\textrm{fair}}}}}
\newcommand{\idealscorefairtxt}{\ensuremath{\textnormal{\textsf{iscore}}_{\textnormal{\textrm{fair}}}}}
\newcommand{\rscore}[1][\relax]{
\def\ArgRscoreI{{#1}}
\RscoreRelay
}%

% \newcommand\RscoreRelay[1][\relax]{%
% \ensuremath{%
%   \realscoretxt^{\ArgRscoreI}%
%   \ifthenelse{\equal{\relax}{#1}}{\relax}{(#1)}%
% }\xspace%
% }

\newcommand\RscoreRelay[1][\relax]{%
\ensuremath{%
    \realscoretxt[\ArgRscoreI]%
    \ifthenelse{\equal{\relax}{#1}}{\relax}{(#1)}%
}\xspace%
}


\newcommand\IscoreRelay[1][\relax]{%
\ensuremath{%
    \idealscoretxt[\ArgIscoreI]%
    \ifthenelse{\equal{\relax}{#1}}{\relax}{(#1)}}\xspace%
}

\newcommand{\rgain}{\ensuremath{\textsc{RealGain}}\xspace}
\newcommand{\iscore}[1][\relax]{
\def\ArgIscoreI{{#1}}
\IscoreRelay
}%

%\newcommand{\mgain}[2][\relax]{\ensuremath{\texttt{iscore}_{#1}^{#2}}\xspace}


\newcommand{\iscorefair}[1][\relax]{
\def\ArgIscoreIfair{{#1}}
\IscorefairRelay
}%
\newcommand\IscorefairRelay[1][\relax]{\ensuremath{\idealscorefairtxt^{\ArgIscoreIfair}(#1)}\xspace}%

\newcommand{\rscorefair}[1][\relax]{
\def\ArgRscoreRfair{{#1}}
\RscorefairRelay
}%
\newcommand\RscorefairRelay[1][\relax]{\ensuremath{\realscorefairtxt^{\ArgRscoreRfair}(#1)}\xspace}%


%\newcommand{\gaintxt}{\ensuremath{\textnormal{\texttt{gain}}}}
%\newcommand{\gaintxt}[1][\relax]{\ensuremath{\hat{U}_R^{#1}}}
\newcommand{\gaintxt}[1][\relax]{\ensuremath{\hat{U}^{#1}}}
\newcommand{\gain}[1][\relax]{
\def\ArgGainI{{#1}}
\GainRelay
}%
\newcommand\GainRelay[1][\relax]{
\ensuremath{\gaintxt[\ArgGainI](#1)}\xspace
}




%\newcommand{\gaingentxt}[1][\prot,\frel]{\ensuremath{\hat{U}_R^{#1}}}
\newcommand{\gaingentxt}[1][\prot,\frel]{\ensuremath{\hat{U}^{#1}}}

\newcommand{\gaingen}[1][\relax]{
\def\ArgGainGenI{{#1}}
\GainGenRelay
}%
\newcommand\GainGenRelay[1][\relax]{
\ifthenelse{\equal{#1}{\relax}}{%
\ensuremath{\gaingentxt[\ArgGainGenI]}
}{%
\ensuremath{\gaingentxt[\ArgGainGenI](#1)}%
}%
\xspace
}

\newcommand{\fcmax}{\ensuremath{f_{\mathrm{max}}}\xspace}
\newcommand{\fgain}[1][\func]{\ensuremath{\textsc{Gain}^{#1}}\xspace}
\newcommand{\mingain}{\ensuremath{{\tt min}\textsc{Gain}}\xspace}
\newcommand{\mfgain}{\ensuremath{\textsc{Gain}^{{\func[SFE]^{\perp}},\vec\gamma}}\xspace}
%\newcommand{\score}{\ensuremath{\textsc{x}}\xspace}
\newcommand{\score}{\ensuremath{v}\xspace}
\newcommand{\utility}{\ensuremath{u}\xspace}
%\newcommand{\score}{X}
\newcommand{\C}{\ensuremath{\mathcal{C}}\xspace}
\newcommand{\attacker}{\ensuremath{{\tt A}}\xspace}
\newcommand{\ug}{\ensuremath{u^{\G}}\xspace}
\newcommand{\designer}{\ensuremath{{\tt D}}\xspace}
\newcommand{\G}{\ensuremath{\mathcal{G}}\xspace}
\newcommand{\negl}{\ensuremath{\lambda}\xspace}
\newcommand{\noti}{\ensuremath{\mu}\xspace}
\newcommand{\itm}{\ensuremath{\mathtt{ITM}}\xspace}
%\newcommand{\iview}{\ensuremath{\mathbb{V}\textsc{iew}}}
\newcommand{\iview}{\ensuremath{\mathbb{V}}}
%\newcommand{\iview}{\ensuremath{\textsc{view}}}
\newcommand{\vcommand}[1]{\cmd{#1}}
\newcommand{\dr}{\ensuremath{\tt DummyRound}\xspace}
\newcommand{\cH}{\mathcal{H}}

\newcommand{\commit}{\ensuremath{\mathtt{commit}}\xspace}
\newcommand{\open}{\mathtt{open}}
\newcommand{\keygen}{\mathtt{keygen}}
\newcommand{\sign}{\mathtt{sign}}
\newcommand{\verify}{\mathtt{verify}}

%\DeclareMathOperator{\gain}{\textsc{gain}}

\newcommand{\mactag}{\mathsf{tag}}
\newcommand{\share}{\mathsf{share}}
\newcommand{\recon}{\mathsf{rec}}


\newcommand{\cR}{\mathcal{R}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}

% Some universal parameters
\newcommand{\parties}{n}
%\newcommand{\secpar}{\ensuremath{\kappa}\xspace}

\newcommand{\rounds}{r}
\newcommand{\random}{R}

\newcommand{\shareset}{S}

\newcommand{\grel}{\langle\mathcal{G}\rangle}
\newcommand{\hrel}{\langle\cH\rangle}

\newcommand{\ith}[1][i]{$#1$-th\xspace}

%\newcommand{\exec}{\textsc{exec}}
%\newcommand{\real}{\textsc{real}}
%\newcommand{\ideal}{\textsc{ideal}}

\newcommand{\diffuse}{\mathcal{F}_{\text{Diffuse}}}
\newcommand{\environ}{\mathcal{Z}}
\newcommand{\receive}{\textsc{Receive}}
\newcommand{\validate}{\textsf{validate}}
\newcommand{\maxval}{\textsf{maxval}}


\makeatletter
\newtheorem*{rep@theorem}{\rep@title}
\newcommand{\newreptheorem}[2]{%
\newenvironment{rep#1}[1]{%
 \def\rep@title{#2 \ref{##1}}%
 \begin{rep@theorem}}%
 {\end{rep@theorem}}}
\makeatother

% \newtheorem{objective}{Objective}
% \newtheorem{lemma}{Lemma}
% \theoremstyle{lemma}
% \newreptheorem{lemma}{Lemma}
% \newtheorem{fact}{Fact}
% \newtheorem{corollary}[lemma]{Corollary}
% \newreptheorem{corollary}{Corollary}
% \newtheorem{theorem}[lemma]{Conjecture}
% \newtheorem{Theorem}{Theorem}
% \newtheorem{Prop}{Proposition}
% \newreptheorem{theorem}{Theorem}
% \newtheorem{claim}{Claim}
% %\theoremstyle{definition}
% \newtheorem{definition}[lemma]{Definition}
% \newtheorem{example}{Example}
% \newtheorem{proposition}[lemma]{Proposition}
%\theoremstyle{remark}
%\newtheorem{remark}{Remark}


%----------llncs----------%
%\spnewtheorem{Theorem}{Theorem}{\bfseries}{\itshape}
\spnewtheorem{Prop}{Proposition}{\bfseries}{\itshape}

% NEW LISTS---------------------------------------------------------------

\newlength{\saveparindent}
\setlength{\saveparindent}{\parindent}
\newlength{\saveparskip}
\setlength{\saveparskip}{\parskip}


\newcounter{ctr}
\newcounter{savectr}
\newcounter{ectr}

\newenvironment{tiret}{%
\begin{list}{\hspace{1pt}\rule[0.5ex]{6pt}{1pt}\hfill}{\labelwidth=15pt%
\labelsep=3pt \leftmargin=18pt \topsep=1pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{1pt}}}{\end{list}}


\newenvironment{newenum}{%
\begin{list}{{\rm \arabic{ctr}.}\hfill}{\usecounter{ctr}\labelwidth=17pt%
\labelsep=6pt \leftmargin=23pt \topsep=.5pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{5pt} }}{\end{list}}

\newenvironment{neweenum}{%
\begin{list}{{\rm \arabic{ctr}.\arabic{ectr}}\hfill}{\usecounter{ectr}%
\labelwidth=28pt\labelsep=4pt \leftmargin=34pt \topsep=0pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{2pt} }}{\end{list}}

\newenvironment{parenum}{%
\begin{list}{{\rm (\arabic{ctr})}\hfill}{\usecounter{ctr}\labelwidth=17pt%
\labelsep=6pt \leftmargin=23pt \topsep=.5pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{5pt} }}{\end{list}}




\newenvironment{venum}{
\begin{list}{{\rm \arabic{ctr}.}\hfill}{\usecounter{ctr}\labelwidth=17pt%
\labelsep=6pt \leftmargin=23pt \topsep=.5pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{1pt} }}{\end{list}}



\newcommand{\ignore}[1]{}  %Ignores inside when typesetting

\newcommand{\todo}[1]{\noindent[\textbf{TODO:} #1]}



\newcommand{\labl}[1]{\textnormal{\textsf{#1}}}

\newcommand{\EvCorr}{\ensuremath{E_\labl{co}}\xspace}
\newcommand{\EvPriv}{\ensuremath{E_\labl{pr}}\xspace}
\newcommand{\EvCrpt}[1][\relax]{E_\labl{cp}^{#1}}

\newcommand{\payCorr}{\ensuremath{\gamma_\labl{co}}\xspace}
\newcommand{\payPriv}{\ensuremath{\gamma_\labl{pr}}\xspace}
\newcommand{\payCrpt}[1][\relax]{\ensuremath{\gamma_\labl{cp}^{#1}}\xspace}

\newcommand{\gmw}[1][\relax]{\ensuremath{\Pi_{\text{GMW}}^{#1}}\xspace}
\newcommand{\cfgn}[1][\relax]{\ensuremath{\Pi_{\text{CFGN}}^{#1}}\xspace}
\newcommand{\iklp}[1][\relax]{\ensuremath{\Pi_{\text{IKLP}}^{#1}}\xspace}
\newcommand{\psfe}[1][\relax]{\ensuremath{\Pi_{\text{Ad-SFE}}^{#1}}\xspace}
\newcommand{\ssfe}[1][\relax]{\ensuremath{\Pi_{\text{St-SFE}}^{#1}}\xspace}
\newcommand{\scoregamma}{\ensuremath{\score^{\vec\gamma}}\xspace}
\newcommand{\vrest}[2]{\ensuremath{#1|_{#2}}\xspace}

\newcommand{\degout}{d^{\textrm{\small{out}}}}
\newcommand{\degin}{d^{\textrm{\small{in}}}}
\newcommand{\neighbout}{\Gamma_1^{\textrm{\small{out}}}}
\newcommand{\neighbin}{\Gamma_1^{\textrm{\small{in}}}}
\newcommand{\distout}{\Gamma^{\textrm{\small{in}}}}
%\newcommand{\graph}{\ensuremath{G}\xspace}
\newcommand{\vset}{\ensuremath{V}\xspace}
\newcommand{\eset}{\ensuremath{E}\xspace}
\newcommand{\bigo}[1][\relax]{\ensuremath{\mathcal{O}(#1)}\xspace}
\newcommand{\polylog}[1][\relax]{\ensuremath{{\sf polylog}(#1)}\xspace}
%\newcommand{\neigh}[1][\relax]{\ensuremath{{\tt Neigh}(#1)}\xspace}
\newcommand{\neigh}[1][\relax]{\ensuremath{{\Gamma}(#1)}\xspace}
\newcommand{\sig}[1][\relax]{\ensuremath{{\tt sig}_{#1}}\xspace}

\newcommand{\ctr}{\textsf{ctr}}
\newcommand{\signkey}{\textsf{sk}}
\newcommand{\vk}{\textsf{vk}}
\newcommand{\prfkey}[1][\relax]{\ensuremath{\textsf{sk}_{#1}}\xspace}
\newcommand{\comm}{\ensuremath{\mathcal{C}}\xspace}
\newcommand{\adaptiveRMT}{\textsf{AdRMT}}
\newcommand{\simu}{\mathcal{S}}

\newcommand{\ncgen}{\mathsf{NCGen}}
\newcommand{\ncenc}{\mathsf{NCEnc}}
\newcommand{\ncdec}{\mathsf{NCDec}}
\newcommand{\ncsim}{\mathsf{NCSim}}


\newcommand{\pk}[1][\relax]{\ensuremath{\textsf{pk}_{#1}}\xspace}
\newcommand{\sk}[1][\relax]{\ensuremath{\textsf{sk}_{#1}}\xspace}

\newcommand{\cpk}[1][\relax]{\ensuremath{\textsf{pk}^\comm_{#1}}\xspace}
\newcommand{\csk}[1][\relax]{\ensuremath{\textsf{s}^\comm_{#1}}\xspace}


\newcommand{\fhepk}[1][\relax]{\ensuremath{\textsf{pk}^{\textrm{FHE}}_{#1}}\xspace}
\newcommand{\fheev}[1][\relax]{\ensuremath{\textsf{ev}^{\textrm{FHE}}_{#1}}\xspace}
 \newcommand{\fhesk}[1][\relax]{\ensuremath{\textsf{sk}^{\textrm{FHE}}_{#1}}\xspace}


\newcommand{\prk}[1][\relax]{\ensuremath{\textsf{sk}_{#1}}\xspace}
%\newcommand{\pcons}[1][\relax]{\ensuremath{\Pi_{\tt Cons}}\xspace}
\newcommand{\pcons}[1][\relax]{\ensuremath{\Pi_{\tt BA}}\xspace}
\newcommand{\pbc}[1][\relax]{\ensuremath{\Pi_{\tt BC}^{#1}}\xspace}
%\newcommand{\pbcRMT}[\relax]{\ensuremath{\Pi_{\tt BC}^{\tt RMT}}\xspace}
\newcommand{\pmpc}[1][\relax]{\ensuremath{\Pi_{\tt MPC}^{#1}}\xspace}

\newcommand{\nextcons}[1][\relax]{\ensuremath{{\tt next}_{\Pi_{\tt
        Cons}}}\xspace}
\newcommand{\hist}{\ensuremath{{\tt hist}}\xspace}

\newcommand{\hidden}{hidden\xspace}
\newcommand{\degree}{\mathsf{deg}}


%===== Macros from the ASIACRYPT paper =====

\newcommand{\Enc}{\ensuremath{{\tt Enc}}\xspace}
\newcommand{\Rec}{\ensuremath{{\tt Rec}}\xspace}
\newcommand{\party}[1]{\ensuremath{^{(#1)}}\xspace}
\newcommand{\tweak}{\ensuremath{T}\xspace}
\newcommand{\xor}{\ensuremath{\oplus}}
\newcommand{\Adv}{\ensuremath{\mathcal{A}}\xspace}
\newcommand{\Env}{\ensuremath{\mathcal{Z}}\xspace}
\newcommand{\edsmt}{\ensuremath{\Func[a-smt]}\xspace}
\newcommand{\bdsmt}{\ensuremath{\Func[$\Delta$-smt]}\xspace}
\newcommand{\fedbc}{\ensuremath{\Func[a-ba]}\xspace}
\newcommand{\Func}[1][\relax]{\ensuremath{\mathcal{F}_{\textsc{#1}}}\xspace}
\newcommand{\Funca}[1][\relax]{\ensuremath{\mathcal{F}^{\rm Asyn}_{\textsc{#1}}}\xspace}
\newcommand{\vfetch}{\ensuremath{\cmd{fetch}}\xspace}
\newcommand{\eom}{\ensuremath{\cmd{eom}}\xspace}
\newcommand{\vactivate}{\ensuremath{\cmd{activate}}\xspace}
\newcommand{\piasfe}{\ensuremath{\pi_{\textsc{a-sfe}}}\xspace}
\newcommand{\pibkr}{\ensuremath{\pi_{\textsc{\tiny BKR}}}\xspace}
\newcommand{\pibkrzo}{\ensuremath{\pi^{0/1}_{\textsc{\tiny BKR}}}\xspace}
%\newcommand{\pibkrzo}{\ensuremath{\pi^{0/1}_{\textrm{BKR}}}\xspace}

\newcommand{\circfsfeprephat}{\ensuremath{C^{F}_{\fprepcirc}}\xspace}
%
%\newtheorem{theorem}{Theorem}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{claim}[theorem]{Claim}
%\newtheorem{definition}{Definition}
%\newtheorem{axiom}[theorem]{Axiom}
%\newtheorem{postulate}{Postulate}
%\theoremstyle{definition}
%\newtheorem{example}{Example}
%\newtheorem{construction}{Construction}
%\theoremstyle{remark}
%\newtheorem{remark}{Remark}
%\newtheorem{fact}[theorem]{Fact}

% LLNCS Class
% \spnewtheorem{fact}{Fact}{\bfseries}{\itshape}
% \newtheorem{fact}{Fact}{\bfseries}{\itshape}

%\newenvironment{nffunc}[3][]{
%\begin{center}
%   \begin{tabular}{|ll|}\hline\small
%     \hspace{.3ex}\begin{minipage}{.97\linewidth}\vspace{0.5ex}
%       {\begin{center}{\bf Functionality} #2 \end{center}}\vspace{-2ex}#3 \begin{itemize}\setlength{\itemsep}{0mm} \setlength{\parskip}{0pt}
% \setlength{\parsep}{0pt}
%\vspace{-1ex}%\vspace{-3ex}
%       }{%
%       \end{itemize}
%       \vspace{-1ex}
%       \smallskip
%     \end{minipage}& \\
%     \hline
%   \end{tabular}
%   \end{center}
%}


\newenvironment{tffbox}{
\begin{figure}[ht!]\small
}{\end{figure}}


% \newenvironment{circdef}[1]
% {
% {
% 	\centering
%
% 	\fbox{
% 		\parbox{13.5cm}{
% 		\begin{large} Circuit #1 \end{large}\vspace{10pt}
%
% }
% {%
% 		}
% 	}
% }
% }


\newenvironment{protdef}[1]
{
	\begin{center}
		\begin{tabular}{|ll|}
			\hline
			\hspace{.3ex}
			\begin{minipage}{.92\linewidth}
				\vspace{0.5ex}
				{\begin{center}{\bf Protocol} #1 \end{center}}
				\vspace{-2ex}
}
{
				\vspace{1ex}
				\smallskip
			\end{minipage}& \\
			\hline
		\end{tabular}
	\end{center}
}

\newenvironment{simdef}[1]
{
	\begin{center}
		\begin{tabular}{|ll|}
			\hline
			\hspace{.3ex}
			\begin{minipage}{.97\linewidth}
				\vspace{0.5ex}
				{\begin{center}{\bf Simulator} #1 \end{center}}
				\vspace{-2ex}
}
{
				\vspace{1ex}
				\smallskip
			\end{minipage}& \\
			\hline
		\end{tabular}
	\end{center}
}

\newcommand{\vSim}[1][\relax]{\ensuremath{\mathcal{S}}\xspace}

% ==== Sandro Macros ====

%\newcommand{\ith}[1]{#1^{\text{th}}}

\newcommand{\field}{\mathbb F}

\newcommand{\bits}{\{0,1\}}

\newcommand{\bit}{\ensuremath{\{0,1\}}} %


\newcommand{\bigoh}[1]{\mathcal O(#1)}

\newcommand{\spara}{\kappa}

\newcommand{\nop}{n}
\newcommand{\noc}{t}
\newcommand{\scirc}{\mathsf{Circ}}

\newcommand{\sigate}[1]{(\mathsf{input},#1)}
\newcommand{\srgate}{(\mathsf{rand})}
\newcommand{\scgate}[3]{(\mathsf{comp},#1,#2,#3)}
\newcommand{\sogate}[2]{(\mathsf{output},#1,#2)}

\newcommand{\sprep}[1]{\textsc{Prepare}_{#1}}

\newcommand{\fsfeprep}{\fsfe{\fprepcirc}}

\newcommand{\phase}{\phi}

\newcommand{\pli}[1]{p_{#1}}

\newcommand{\etal}{\emph{et al.}}

\newenvironment{packedenum}{
\begin{enumerate}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{enumerate}}

\newenvironment{packeditem}{
\begin{itemize}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{itemize}}

\newenvironment{indentpar}[1]
{\begin{list}{}
         {\setlength{\leftmargin}{#1}}
         \item[]
}
{\end{list}}

\newcommand{\senc}[2]{\mathsf{Enc}_{#1}\left(#2\right)}
\newcommand{\sdec}[2]{\mathsf{Dec}_{#1}\left(#2\right)}


%\newcommand{\sinput}{\ensuremath{\cmd{input}}\xspace}
\newcommand{\soutput}{\ensuremath{\cmd{output}}\xspace}

\newcommand{\sphase}{\phi}


% === Circuits ===
\newcommand{\crc}{C}

\newcommand{\crcinp}[1]{{b_{#1}}}

\newcommand{\crcli}{\alpha}
\newcommand{\crcri}{\beta}
\newcommand{\crco}{\gamma}

\newcommand{\crclig}[1]{{\alpha_{#1}}}
\newcommand{\crcrig}[1]{{\beta_{#1}}}
\newcommand{\crcog}[1]{{\gamma_{#1}}}

\newcommand{\crcg}{g}
\newcommand{\crcw}{\omega}


% === Garbled Circuits ===
\newcommand{\gcminp}[1]{{z_{#1}}}
\newcommand{\gcmw}[1]{{m_{#1}}}
\newcommand{\vsgcmw}[1]{{\vs{m}_{#1}}}

\newcommand{\gcft}[1]{{T_{#1}}}
\newcommand{\vsgcft}[1]{{\vs{T}_{#1}}}
\newcommand{\gcftr}[3]{{t^{#2#3}_{#1}}}
\newcommand{\vsgcftr}[3]{{\vs{t}^{#2#3}_{#1}}}
\newcommand{\gcsftr}[4]{{t^{#2#3,#4}_{#1}}}

\newcommand{\gcgft}[1]{{C_{#1}}}
\newcommand{\vsgcgft}[1]{{\vs{C}_{#1}}}
\newcommand{\gcgftr}[3]{{c^{#2#3}_{#1}}}
\newcommand{\gcsgft}[2]{{C_{#1}^{#2}}}
\newcommand{\vsgcsgft}[2]{{\vs{C}_{#1}^{#2}}}
\newcommand{\gcsgftr}[4]{{c^{#2#3,#4}_{#1}}}
\newcommand{\vsgcsgftr}[4]{{\vs{c}^{#2#3,#4}_{#1}}}

\newcommand{\gcz}[2]{{z^{#1#2}}}
\newcommand{\gczw}[3]{{z^{#2#3}_{#1}}}
\newcommand{\vsgczw}[3]{{\vs{z}^{#2#3}_{#1}}}



\newcommand{\gck}[2]{{k_{#1,#2}}}
\newcommand{\vsgcsk}[3]{{\vs{k}_{#1,#2}^{#3}}}
\newcommand{\gcsk}[3]{{k_{#1,#2}^{#3}}}
\newcommand{\gcik}[1]{{k_{#1}}}
\newcommand{\vsgcik}[1]{{\vs{k}_{#1}}}
\newcommand{\gcisk}[2]{{k_{#1}^{#2}}}
\newcommand{\vsgcisk}[2]{{k_{#1}^{#2}}}


\newcommand{\dictk}{{\kappa}}
\newcommand{\dictz}{{\zeta}}

\newcommand{\dictke}[2]{{\dictk(#1,#2)}}
\newcommand{\dictze}[1]{{\dictz(#1)}}

% \newcommand{\xor}{\hspace{5pt} \mathtt{XOR} \hspace{5pt}}
\newcommand{\nand}{\hspace{3pt} \mathtt{NAND} \hspace{3pt}}
\newcommand{\nandc}{\mathtt{NAND}}

\newcommand{\enc}[4]{\mathsf{Enc}^{#4}_{#1,#2}\left(#3\right)}
%\newcommand{\dec}[4]{\mathsf{Dec}^{#4}_{#1,#2}\left(#3\right)}

\newcommand{\sharing}[1]{{[#1]}}
%\newcommand{\share}[2]{{[#1]_{#2}}}

\newcommand{\prepcirc}{\mathsf{Prep}}
\newcommand{\fprepcirc}{f_\textsc{prep}^\scirc}

\newcommand{\degrees}{$^\circ$}
\newcommand{\microns}{$\mu$m$\;$}

\newcommand{\ket}[1]{|#1\rangle}
\newcommand{\bra}[1]{\langle #1|}
\newcommand{\bool}{\{0,1\}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\idop}{\mathcal{I}}

\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}

\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}

\newcommand{\cZ}{\mathcal{Z}}


\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbZ}{\mathbb{Z}}


% --------- math new -----%
\mdfsetup{skipabove=2ex,skipbelow=10pt}

\mdfdefinestyle{figstyle}{ %
  linecolor=black!7, %
  backgroundcolor=black!7, %
  innertopmargin=10pt, %
  innerleftmargin=25pt, %
  innerrightmargin=25pt, %
  innerbottommargin=10pt
}


\renewenvironment{protocol}{
  \begin{mdframed}[style=figstyle]}{
  \end{mdframed}}

\newcommand{\I}{\ensuremath{\mathcal{I}}}
\newcommand{\mrsearch}{\ensuremath{k}\textsc{-BerSearch}}
\newcommand{\samp}{\textsf{Samp}} \newcommand{\powt}{\eta}
\newcommand{\stdbo}{\textsf{StdBO}} \newcommand{\fpbo}{\textsf{FPhBO}}
\newcommand{\vx}{\mathbf{x}} \newcommand{\vy}{\mathbf{y}}
\newcommand{\vz}{\mathbf{z}} \newcommand{\pvx}{{\bar{\mathbf{x}}}}
\newcommand{\tvx}{{\tilde{\mathbf{x}}}}
\newcommand{\aproj}{\mathbf{\Pi}} % success projection
\newcommand{\dproj}{\mathbf{P}} % database projection
\newcommand{\bpara}{\ensuremath{\eta}} %
\newcommand{\beru}{\ensuremath{\mathcal{U}_\bpara}} %
\newcommand{\cquery}{\ensuremath{\tau_c}} %
\newcommand{\qquery}{\ensuremath{\tau_q}} %
\newcommand{\aquery}{\ensuremath{\tau}} % aggregate query
\newcommand{\errp}{\ensuremath{\varepsilon}} %
\newcommand{\fnull}{\ensuremath{f_{\emptyset}}} %
\newcommand{\expt}{\ensuremath{\mathbb{E}}} %
\newcommand{\advan}{\textsf{ADV}} %
\newcommand\norm[1]{\left\lVert#1\right\rVert}

%\renewcommand{\secpar}{\ensuremath{\lambda}\xspace}


\newcommand{\berunit}{\ensuremath{\mathcal{U}_p}}



\DeclareGraphicsRule{.tif}{png}{.png}{`convert #1 `dirname #1`/`basename #1 .tif`.png}


%-----------new commands FS---------%
\newcommand{\cprim}[1]{\textup{\textsf{#1}}} % primitives
\newcommand{\dsearch}{\cprim{Dist-Search}} % D-search

\newcommand{\uniqunifsearch}{\cprim{Unique-Uniform-Search}} % D-search


\newcommand{\ff}{\ensuremath{\mathcal{F}}} % 
\newcommand{\ffunc}{\ensuremath{\left\{ f: X \to \bits \right\}}} % ffunc
\newcommand{\distr}{\ensuremath{{D}}} % distr
\newcommand{\solnl}{\ensuremath{\nu_\distr}} % likelihood of soln
\newcommand{\specnorm}[1]{\left\| #1 \right\|} % spectral norm
\newcommand{\dadv}[2]{\Delta_{#1,#2}} % distinguish advantage
\newcommand{\ho}[1]{\left[{#1}\right]} % hybrid oracle
\newcommand{\berpar}{\ensuremath{\eta}} % bernoulli parameter
\newcommand{\pfail}{\ensuremath{\delta}} % failure prob
\newcommand{\succp}{{\mathsf{Succ}}} % succ prob
\newcommand{\tproj}{\ensuremath{\gamma}} % intermediate proj
\newcommand{\identity}{\mathds{1}}
\newcommand{\qoracle}{\ensuremath{Q}}
\newcommand{\coracle}{\ensuremath{P}} 

% Problems names

\newcommand{\mwunif}{\textbf{$(\mathsf{M}, \mathsf{w}$)-Uniform Search}}


\newcommand{\mwfix}{\textbf{Fixed-$(\mathsf{M}, \mathsf{w}$) Search}}



\newcommand{\hybrid}{hybrid classical-quantum}


\newcommand{\probfailunif}{p_{\mathsf{unif-fail}}}

\newcommand{\probfailfix}{p_{\mathsf{fix-fail}}}


% HASH FUNCTIONS DEFS

\newcommand{\qpt}{\mathsf{QPT}}


\newcommand{\ow}{\mathsf{OW}} %

\newcommand{\smow}{\mathsf{SM_p-OW}} %

\newcommand{\mmow}{\mathsf{MM_p-OW}} %

%%%%
\newcommand{\spr}{\mathsf{SPR}} %
\newcommand{\smspr}{\mathsf{SM_p-SPR}} %
\newcommand{\mmspr}{\mathsf{MM_p-SPR}} %

%%%%
\newcommand{\etcr}{\mathsf{eTCR}} %
\newcommand{\smetcr}{\mathsf{SM_p-eTCR}} %
\newcommand{\mmetcr}{\mathsf{MM_p-eTCR}} %

%\newcommand{\succ}{\mathsf{Succ}} %



%% BACKBONE DEFS

\def\chain{\mathcal{C}}
\newcommand{\pow}{\text{PoW}} %
\newcommand{\pows}{\text{PoWs}} %

\newcommand{\chainpow}{\textsc{Chain-of-PoWs}}


\newcommand{\hyb}{\mathsf{hyb}} %



\newcommand{\majority}{\mathsf{majority}} %

\newcommand{\hw}{\mathsf{hw}} %


\DeclareMathOperator*{\argmax}{arg\,max}


\newcommand{\weight}{\omega}


\newcommand{\newd}[1]{{\tilde #1}}

